Narrowest-Over-Threshold Detection of Multiple Change-points and Change-point-like Features

We propose a new, generic and flexible methodology for nonparametric function estimation, in which we first estimate the number and locations of any features that may be present in the function, and then estimate the function parametrically between each pair of neighbouring detected features. Examples of features handled by our methodology include change-points in the piecewise-constant signal model, kinks in the piecewise-linear signal model, and other similar irregularities, which we also refer to as generalised change-points. Our methodology works with only minor modifications across a range of generalised change-point scenarios, and we achieve such a high degree of generality by proposing and using a new multiple generalised change-point detection device, termed Narrowest-Over-Threshold (NOT). The key ingredient of NOT is its focus on the smallest local sections of the data on which the existence of a feature is suspected. Crucially, this adaptive localisation technique prevents NOT from considering subsamples containing two or more features, a key factor that ensures the general applicability of NOT. For selected scenarios, we show the consistency and near-optimality of NOT in detecting the number and locations of generalised change-points. Furthermore, we propose to select NOT's threshold (automatically) via the strengthened Schwarz Information Criterion (sSIC) and give theoretical justifications. The NOT estimators are easy to implement and rapid to compute: the entire threshold-indexed solution path can be computed in close-to-linear time. Importantly, the NOT approach is easy to extend by the user to tailor to their own needs. There is no single competitor, but we show that the performance of NOT matches or surpasses the state of the art in the scenarios tested. Our methodology is implemented in the R package \textbf{not}.

==> tables/gbp_usd_changepoints_nmcd.tex <==
 9 September 2008 &  \\ 
  31 March 2009 &  \\ 
  4 August 2009 &  \\ 
  17 January 2012 &  \\ 
  26 February 2015 &  \\ 
  15 June 2016 &  \\ 
  

==> tables/gbp_usd_changepoints_not.tex <==
 2 January 2004 &  \\ 
  27 May 2004 &  \\ 
  11 September 2008 &  \\ 
  2 April 2009 &  \\ 
  11 January 2012 &  \\ 
  14 February 2014 &  \\ 
  29 August 2014 &  \\ 
  16 June 2016 &  \\ 
  

==> tables/oil_price_changepoints_nmcd.tex <==
 28 August 2008 &  \\ 
  22 January 2009 &  \\ 
  23 October 2009 &  \\ 
  12 October 2012 &  \\ 
  1 October 2014 &  \\ 
  21 January 2016 &  \\ 
  22 February 2016 &  \\ 
  

==> tables/oil_price_changepoints_not.tex <==
 28 April 2003 &  \\ 
  1 September 2008 &  \\ 
  12 January 2009 &  \\ 
  1 October 2009 &  \\ 
  12 November 2012 &  \\ 
  30 September 2014 &  \\ 
  5 January 2016 &  \\ 
  

==> tables/temp_anomalies_changepoints.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{ll}
  \hline
date & comment \\ 
  \hline
March 1901 &  \\ 
  December 1910 &  \\ 
  July 1915 &  \\ 
  June 1935 &  \\ 
  April 1944 &  \\ 
  December 1946 &  \\ 
  June 1976 &  \\ 
  May 2015 &  \\ 
   \hline
\end{tabular}
\caption{\label{Table:temp_anomalies_changepoints}: Change-point detected using NOT SIC methodology in the temperature anomalies data.} 
\end{table}

